Restructuring Conversations using Discourse Relations for Zero-shot Abstractive Dialogue Summarization

Dialogue summarization is a challenging problem due to the informal and unstructured nature of conversational data. Recent advances in abstractive summarization have been focused on data-hungry neural models and adapting these models to a new domain requires the availability of domain-specific manually annotated corpus created by linguistic experts. We propose a zero-shot abstractive dialogue summarization method that uses discourse relations to provide structure to conversations, and then uses an out-of-the-box document summarization model to create final summaries. Experiments on the AMI and ICSI meeting corpus, with document summarization models like PGN and BART, shows that our method improves the ROGUE score by up to 3 points, and even performs competitively against other state-of-the-art methods.

==> tables/discourse.tex <==
\begin{table}
\centering
\scriptsize
\caption{Example for Discourse Rearrangement}
\label{tab:discourse}
\begin{tabular}{|l|c|}
\hline 
\textbf{Example Dialogue \#1} & \textbf{Dialogue Acts} \\ 
\hline
S1 :  Is S2 ready? & Yes-No-Question \\
S3 : I am packing my bag. & Statement \\
S2 : Yes. & Yes answers \\
\hline
\multicolumn{2}{|l|}{\textbf{Generated Paragraph} : S1 asked is S2 ready} \\
\multicolumn{2}{|l|}{and S2 agreed. S3 said I am packing my bag.} \\
\hline
\hline
% \textbf{Example Dialogue \#2} & \textbf{Dialogue Acts} \\
% \hline
% S1 : Why do you think gay marriages are banned? & Wh-Question \\
% S2 : I think the reason for gay marriages being banned is not entirely & Affirmative non-yes answers \\
% political. & \\
% \hline
% \multicolumn{2}{|l|}{\textbf{Generated Paragraph} : S1 asked why does S2 think gay marriages are banned and S2 replied S2} \\
% \multicolumn{2}{|l|}{thinks the reason for gay marriages being banned is not entirely political.} \\
% \hline
% \hline

% \textbf{Example Dialogue \#2} & \textbf{Dialogue Acts} \\
% \hline
% S1 : Why do you think gay marriages are banned? & Wh-Question \\
% S2 : I think the reason for ban is not entirely political & Affirmative non-yes answers \\
% \hline
% \multicolumn{2}{|l|}{\textbf{Generated Paragraph} : S1 asked why does S2 think gay marriages are banned and S2 replied S2} \\
% \multicolumn{2}{|l|}{think the reason for ban is not entirely political.} \\
% \hline
% \hline

\textbf{Example Dialogue \#2} & \textbf{Dialogue Acts} \\ 
\hline
S1 : I am going for a walk. & Statement-\\
& non-opinion \\
S2 : Oh, Okay. & Acknowledge \\
\hline
\multicolumn{2}{|l|}{\textbf{Generated Paragraph} : S1 said S1 is going  } \\
\multicolumn{2}{|l|}{for a walk and S2 acknowledged.} \\
\hline
\end{tabular}
\end{table}

==> tables/results_argumentative.tex <==
\begin{table}
\centering
\small
\setlength\tabcolsep{4pt}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline 
\multicolumn{1}{|c|}{\textbf{Method}} & \multicolumn{3}{|c|}{\textbf{ROGUE-1}} & \multicolumn{3}{|c|}{\textbf{ROGUE-2}} \\
\cline{2-7}
  & \textbf{R} & \textbf{P} & \textbf{F1} & \textbf{R} & \textbf{P} & \textbf{F1} \\
\hline
PGN & 30.15 & 25.51 & 27.45 & 4.71 & 3.99 & 4.30 \\
\cline{2-7}
+ AR & 34.91 & 28.64 & 31.23 & 7.71 & 6.33 & 6.91 \\
\cline{2-7}
+ CF + DR & 46.49 & 38.38 & 41.76 & 12.62 & 10.53 & 11.4 \\
\hline
BART & 30.15 & 25.51 & 27.45 & 4.71 & 3.99 & 4.30 \\
\cline{2-7}
+ AR & 34.91 & 28.64 & 31.23 & 7.71 & 6.33 & 6.91 \\
\cline{2-7}
+ CF + DR & 46.49 & 38.38 & 41.76 & 12.62 & 10.53 & 11.4 \\
\hline
\end{tabular}
\caption{Internal ablation study on the Argumentative Dialogue Summary Corpus}
\label{tab:argumentative}
\end{table}

